Zero-shot Blind Image Denoising via Implicit Neural Representations

Recent denoising algorithms based on the "blind-spot" strategy show impressive blind image denoising performances, without utilizing any external dataset. While the methods excel in recovering highly contaminated images, we observe that such algorithms are often less effective under a low-noise or real noise regime. To address this gap, we propose an alternative denoising strategy that leverages the architectural inductive bias of implicit neural representations (INRs), based on our two findings: (1) INR tends to fit the low-frequency clean image signal faster than the high-frequency noise, and (2) INR layers that are closer to the output play more critical roles in fitting higher-frequency parts. Building on these observations, we propose a denoising algorithm that maximizes the innate denoising capability of INRs by penalizing the growth of deeper layer weights. We show that our method outperforms existing zero-shot denoising methods under an extensive set of low-noise or real-noise scenarios.

==> contents/3_inr_deeper.tex <==
\subsection{Deeper layers of INR} \label{ssec:exp_layer}


We seek to strengthen the inductive bias of INR further by exploiting the properties of INR architecture. Here, we focus on the difference in the roles that neurons in different layers play. For this purpose, we examine the features generated by neurons in each layer. More specifically, we select a neuron in each layer and measure the activation of the neuron corresponding to each coordinate values as an input. This procedure allows us to track the change in a subnetwork output as the training proceeds.

We provide the visualization of these features in \cref{fig:implicit_features}, where we analyze an INR with four hidden layers trained on a noisy image. We report the features for both (a) INR trained until convergence, and (b) INR stopped at the optimal early stopping iteration (in terms of clean-image PSNR). From the figure, we observe a hierarchy of features; earlier layer neurons mainly represent low-frequency patterns while latter layer neurons generate fine-grained details. One notable difference between the fully-trained and early-stopped model is the behavior of latter-layer neurons. In particular, we observe that after the optimal early stopping epoch, several latter layer neurons tend to fit the white noise, instead of the pattern relevant to the clean image. In contrast, visualizations of earlier layer neurons remain similar (we note that a similar finding has been reported by \citet{chen2021featurematching}, where the authors use the smooth interpolation of implicit features for 3D shape deformation). This motivates us to constrain the growth of latter-layer weights via selective weight decay, which is what we do in the proposed denoising method.




==> figuretexs/f2.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/psnr_plot}
\caption{The inductive architectural bias of INR. We fit an INR to an image injected with the Gaussian noise and compare the PSNR of the INR-generated with both the clean image (orange) and the noisy image (blue). INR fits the clean image first, and the noisy image later.}
\label{fig:psnr_plot}
\vspace{-1em}
\end{figure}

==> figuretexs/f4.tex <==
\begin{figure*}[ht]
\centering
\subfloat[Signal and Noise Impedances of DIP] {\includegraphics[width=1.05\columnwidth]{figures/DIP_reluctancy}}\subfloat[Signal and Noise Impedances of INR] {\includegraphics[width=1.05\columnwidth]{figures/INR_reluctancy}}
\caption{Learning curve on clean image (blue), images contaminated with additive Gaussian noise (orange for $\sigma = 25$ and green for $\sigma=50$) and white noise (red). The learning curve for INR converges faster on a clean image.}
\label{fig:reluctance_plot}
\end{figure*}

==> tables/ablation.tex <==
\begin{table}[t]
\caption{Effect of weight decay conditional to the depth of INR. We denoise \textit{House.png} image in Set9 with hyperparameter $\lambda=0.1$ for weight decay. Regularization improves PSNR(dB) for INR with more than 5 hidden layers.
}\label{ablation}
\centering
\begin{tabular}{@{}ccc@{}}
\toprule
INR  & w/o weight decay & w/ weight decay\\
\midrule
4 hidden layers & \textbf{30.60} & 29.24 \\
5 hidden layers & 31.15 & \textbf{31.39} \\
6 hidden layers & 31.41 & \textbf{31.72}\\
7 hidden layers & 31.49 & \textbf{31.85} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/inductive_bias.tex <==
\begin{table*}[t]
\caption{Per-image denoising performance. The denoising result of each architecture empirically proves the spectral bias of DIP and INR. The \textbf{bold} indicates the best results.}
\label{tab:spectralbias_psnr}
\centering
\scalebox{1}{
\begin{tabular}{c|c|cc|cc}
\toprule
Image & DIP & DIP Linear-128 & DIP Linear-2048 & INR-ReLU & \textbf{INR-SIREN}\\
\midrule
Baboon & 24.73 & 20.48 & 20.35 & 24.56 & \textbf{24.85}\\
F16 & 27.00 & 20.72 & 18.60 & 26.67 & \textbf{30.10}\\
House & 26.89 & 20.69 & 18.89 & 27.21 & \textbf{28.90}\\
Kodim01 & 25.90 & 20.35 & 20.54 & 25.95 & \textbf{27.32}\\
Kodim02 & 29.20 & 20.74 & 20.59 & 29.99 &\textbf{29.65}\\
Kodim03 & 29.26 & 20.47 & 18.13 & 29.62 & \textbf{30.77}\\
Kodim12 & 29.61 & 20.36 & 17.74 & 29.63 & \textbf{30.34}\\
Lena & 27.49 & 20.48 & 18.67 & 27.78 & \textbf{30.45}\\
Peppers & 27.12 & 20.60 & 18.98 & 26.82 & \textbf{29.56}\\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/peak_time.tex <==
\begin{table}[t]
\caption{Peak PSNR (and the corresponding epoch) of DIP and INR for denoising a single image from the CBSD dataset, under various noise levels. INR reaches the peak PSNR in fewer iterations. \textbf{Bold} indicates higher PSNR and faster learning of clean prior.
}
\label{tab:peak_time}
\begin{center}
\begin{tabular}{@{}ccc@{}}
\toprule
Noise Level & DIP & INR \\
\midrule
$\sigma=5$ & 34.105 (5935) & \textbf{37.817 (3917)} \\
$\sigma=10$ & 32.311 (4725) & \textbf{32.954 (1710)} \\
$\sigma=15$ & 30.377 (2326) & \textbf{30.437 (1096)} \\
$\sigma=20$ & \textbf{27.843} (643) & 27.830 \textbf{(637)} \\
$\sigma=25$ & 26.162 (875) & \textbf{26.303 (461)}\\
\bottomrule
\end{tabular}
\end{center}
\end{table}
